SoK: DARPA's AI Cyber Challenge (AIxCC): Competition Design, Architectures, and Lessons Learned

DARPA's AI Cyber Challenge (AIxCC, 2023--2025) is the largest competition to date for building fully autonomous cyber reasoning systems (CRSs) that leverage recent advances in AI -- particularly large language models (LLMs) -- to discover and remediate vulnerabilities in real-world open-source software. This paper presents the first systematic analysis of AIxCC. Drawing on design documents, source code, execution traces, and discussions with organizers and competing teams, we examine the competition's structure and key design decisions, characterize the architectural approaches of finalist CRSs, and analyze competition results beyond the final scoreboard. Our analysis reveals the factors that truly drove CRS performance, identifies genuine technical advances achieved by teams, and exposes limitations that remain open for future research. We conclude with lessons for organizing future competitions and broader insights toward deploying autonomous CRSs in practice.

==> tbl/sarif-techniques.tex <==
{\rowcolors{2}{}{gray!15}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\begin{table*}[t]
\centering
\caption{SARIF Validation Techniques Across Teams.}
\label{t:sarif-techniques}
\smaller
\setlength{\tabcolsep}{4pt}
\adjustbox{trim=0pt 0pt 3pt 0pt,clip,max width=\textwidth}{
\begin{tabular}{@{}>{\cellcolor{white}}c L{2.0cm} L{1.72cm}L{1.72cm}L{1.72cm}L{1.72cm}L{1.72cm}L{1.72cm}L{1.72cm}@{}}
  \toprule
  & & \hyperlink{team:AT}{\texttt{AT}} & \hyperlink{team:TB}{\texttt{TB}} & \hyperlink{team:TI}{\texttt{TI}} & \hyperlink{team:FB}{\texttt{FB}} & \hyperlink{team:SP}{\texttt{SP}} & \hyperlink{team:42}{\texttt{42}} & \hyperlink{team:LC}{\texttt{LC}} \\
  \midrule
  & Category & PoV-centric & PoV-centric & Bug-cand-centric & PoV-centric & LLM-judge-centric & LLM-judge-centric & LLM-judge-centric \\
  & Implementation$^*$ & LLM-Based & Heuristic-Based & LLM-Based & Heuristic-Based; LLM-Based & LLM-Based & LLM-Based & LLM-Based \\
  \multirow{-4}{*}{\parbox{1.4cm}{\centering\textbf{Validation Strategy}}}
  & Pre-validation Sanity Check$^\dagger$ & Format; File; Function; Line no. & Format & Format & Format & Format; File; Function & File; Function; Line no. & \X \\
  \midrule
  & SARIF Report & Full Report & File; Function; StartLine; EndLine & Function; File; Description; Rule & File; StartLine; EndLine; Rule; Message & Function; File; StartLine; Rule; Message & Full Report & Full Report \\
  & PoV/Bug Cand Info & Crash Log; Patch Diff (if available) & StackTrace (File; Function; Line) & Function; File; Description; Condition & Partial Crash Log (StackTrace; Error Message) & N/A & Crash Log & N/A \\
  \multirow{-6}{*}{\parbox{1.4cm}{\centering\textbf{Used Inputs for Validation}}}
  & Code Context & Surrounding Context; Dynamic Retrieval$^\ddagger$ & \X & \X & Enclosing Function & Dynamic Retrieval & Dynamic Retrieval & Surrounding Context \\
  \bottomrule
\end{tabular}
}
\\[2pt]
\raggedright
{\footnotesize
$^*$ Heuristic-based follows developer-defined workflows; LLM-based relies on LLM queries.\\
$^\dagger$ Verifies SARIF report format and checks whether referenced artifacts (files, functions or lines) exist before main validation.\\
$^\ddagger$ Additional code context dynamically requested by LLM.
}
\end{table*}
}


==> tbl/vuln_sarif_details/cpvs.tex <==
\onecolumn
\begin{longtblr}[
  caption = {CPV (Challenge Problem Vulnerability) details. $\square$ indicates full-mode challenges, $\blacktriangle$ indicates delta-mode challenges.},
  label = {t:cpv-details},
]{
  colspec = {c|l|llllX[l]},
  rows = {font=\scriptsize, abovesep=0pt, belowsep=-1pt},
  row{1} = {font=\bfseries\scriptsize, belowsep=1pt},
  rowhead = 1,
  colsep = 3pt,
}
\toprule\addlinespace[2pt]
Lang & Ph & Project & ID & Vuln & CWE & CWE Name \\
\midrule
\SetCell[r=43]{m} \textbf{C} & \SetCell[r=26]{} P2 & libavif & \SetCell{bg=gray!15} \cc{av2$\blacktriangle$02} & \SetCell{bg=gray!15} avif-002 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/126.html}{126} & \SetCell{bg=gray!15} Buffer Over-read \\
\cline{3-7}
 &  & \SetCell[r=2]{} little-cms & \cc{cm1$\square$01} & lcms-001 & \href{https://cwe.mitre.org/data/definitions/476.html}{476} & NULL Pointer Dereference \\
 &  &  & \SetCell{bg=gray!15} \cc{cm1$\square$02} & \SetCell{bg=gray!15} lcms-002 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/126.html}{126} & \SetCell{bg=gray!15} Buffer Over-read \\
\cline{3-7}
 &  & \SetCell[r=6]{} curl & \cc{cu2$\blacktriangle$06} & curl-006 & \href{https://cwe.mitre.org/data/definitions/476.html}{476} & NULL Pointer Dereference \\
 &  &  & \SetCell{bg=gray!15} \cc{cu3$\blacktriangle$07} & \SetCell{bg=gray!15} curl-007 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/476.html}{476} & \SetCell{bg=gray!15} NULL Pointer Dereference \\
 &  &  & \cc{cu4$\blacktriangle$03} & curl-003 & \href{https://cwe.mitre.org/data/definitions/121.html}{121} & Stack-based Buffer Overflow \\
 &  &  & \SetCell{bg=gray!15} \cc{cu4$\blacktriangle$08} & \SetCell{bg=gray!15} curl-008 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/476.html}{476} & \SetCell{bg=gray!15} NULL Pointer Dereference \\
 &  &  & \cc{cu5$\blacktriangle$01} & curl-001 & \href{https://cwe.mitre.org/data/definitions/134.html}{134} & Use of Externally-Controlled Format String \\
 &  &  & \SetCell{bg=gray!15} \cc{cu5$\blacktriangle$02} & \SetCell{bg=gray!15} curl-002 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/787.html}{787} & \SetCell{bg=gray!15} Out-of-bounds Write \\
\cline{3-7}
 &  & \SetCell[r=2]{} libexif & \cc{ex2$\blacktriangle$01} & exif-001 & \href{https://cwe.mitre.org/data/definitions/122.html}{122} & Heap-based Buffer Overflow \\
 &  &  & \SetCell{bg=gray!15} \cc{ex3$\blacktriangle$02} & \SetCell{bg=gray!15} exif-002 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/121.html}{121} & \SetCell{bg=gray!15} Stack-based Buffer Overflow \\
\cline{3-7}
 &  & freerdp & \cc{fp2$\blacktriangle$02} & vuln\_002 & \href{https://cwe.mitre.org/data/definitions/122.html}{122} & Heap-based Buffer Overflow \\
\cline{3-7}
 &  & libxml2 & \SetCell{bg=gray!15} \cc{lx3$\blacktriangle$04} & \SetCell{bg=gray!15} vuln\_004 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/122.html}{122} & \SetCell{bg=gray!15} Heap-based Buffer Overflow \\
\cline{3-7}
 &  & \SetCell[r=4]{} mongoose & \cc{mg1$\blacktriangle$01} & mongoose\_1 & \href{https://cwe.mitre.org/data/definitions/121.html}{121} & Stack-based Buffer Overflow \\
 &  &  & \SetCell{bg=gray!15} \cc{mg2$\blacktriangle$02} & \SetCell{bg=gray!15} mongoose\_2 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/125.html}{125} & \SetCell{bg=gray!15} Out-of-bounds Read \\
 &  &  & \SetCell[r=2]{} \cc{mg1$\square$00} & \SetCell[r=2]{} mongoose\_0 & \href{https://cwe.mitre.org/data/definitions/121.html}{121} & Stack-based Buffer Overflow \\
 &  &  &  &  & \href{https://cwe.mitre.org/data/definitions/193.html}{193} & Off-by-one Error \\
\cline{3-7}
 &  & \SetCell[r=5]{} shadowsocks-libev & \SetCell{bg=gray!15} \cc{ss1$\square$00} & \SetCell{bg=gray!15} shadowsocks-libev\_0 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/126.html}{126} & \SetCell{bg=gray!15} Buffer Over-read \\
 &  &  & \cc{ss1$\square$01} & shadowsocks-libev\_1 & \href{https://cwe.mitre.org/data/definitions/126.html}{126} & Buffer Over-read \\
 &  &  & \SetCell{bg=gray!15} \cc{ss1$\square$02} & \SetCell{bg=gray!15} shadowsocks-libev\_2 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/126.html}{126} & \SetCell{bg=gray!15} Buffer Over-read \\
 &  &  & \cc{ss1$\square$03} & shadowsocks-libev\_3 & \href{https://cwe.mitre.org/data/definitions/126.html}{126} & Buffer Over-read \\
 &  &  & \SetCell{bg=gray!15} \cc{ss1$\square$04} & \SetCell{bg=gray!15} shadowsocks-libev\_4 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/126.html}{126} & \SetCell{bg=gray!15} Buffer Over-read \\
\cline{3-7}
 &  & \SetCell[r=4]{} systemd & \cc{sd1$\square$01} & systemd-001 & \href{https://cwe.mitre.org/data/definitions/787.html}{787} & Out-of-bounds Write \\
 &  &  & \SetCell{bg=gray!15} \cc{sd1$\square$03} & \SetCell{bg=gray!15} systemd-003 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/122.html}{122} & \SetCell{bg=gray!15} Heap-based Buffer Overflow \\
 &  &  & \cc{sd1$\square$04} & systemd-004 & \href{https://cwe.mitre.org/data/definitions/415.html}{415} & Double Free \\
 &  &  & \SetCell{bg=gray!15} \cc{sd1$\square$05} & \SetCell{bg=gray!15} systemd-005 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/415.html}{415} & \SetCell{bg=gray!15} Double Free \\
\hline
 & \SetCell[r=9]{} P3 & dav1d & \cc{da1$\square$01} & dav1d-001 & \href{https://cwe.mitre.org/data/definitions/190.html}{190} & Integer Overflow or Wraparound \\
\cline{3-7}
 &  & \SetCell[r=8]{} wireshark & \SetCell{bg=gray!15} \cc{ws1$\square$01} & \SetCell{bg=gray!15} vuln\_001 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/121.html}{121} & \SetCell{bg=gray!15} Stack-based Buffer Overflow \\
 &  &  & \cc{ws1$\square$02} & vuln\_002 & \href{https://cwe.mitre.org/data/definitions/416.html}{416} & Use After Free \\
 &  &  & \SetCell{bg=gray!15} \cc{ws1$\square$05} & \SetCell{bg=gray!15} vuln\_005 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/134.html}{134} & \SetCell{bg=gray!15} Use of Externally-Controlled Format String \\
 &  &  & \cc{ws1$\square$10} & vuln\_010 & \href{https://cwe.mitre.org/data/definitions/122.html}{122} & Heap-based Buffer Overflow \\
 &  &  & \SetCell[r=3]{bg=gray!15} \cc{ws1$\square$11} & \SetCell[r=3]{bg=gray!15} vuln\_011 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/121.html}{121} & \SetCell{bg=gray!15} Stack-based Buffer Overflow \\
 &  &  &  &  & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/122.html}{122} & \SetCell{bg=gray!15} Heap-based Buffer Overflow \\
 &  &  &  &  & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/680.html}{680} & \SetCell{bg=gray!15} Integer Overflow to Buffer Overflow \\
 &  &  & \cc{ws1$\square$12} & vuln\_012 & \href{https://cwe.mitre.org/data/definitions/457.html}{457} & Use of Uninitialized Variable \\
\hline
 & \SetCell[r=1]{} P4 & freerdp & \SetCell{bg=gray!15} \cc{fp3$\blacktriangle$03} & \SetCell{bg=gray!15} vuln\_003 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/123.html}{123} & \SetCell{bg=gray!15} Write-what-where Condition \\
\hline
 & \SetCell[r=7]{} P7 & \SetCell[r=6]{} wireshark & \cc{ws1$\blacktriangle$03} & vuln\_003 & \href{https://cwe.mitre.org/data/definitions/787.html}{787} & Out-of-bounds Write \\
 &  &  & \SetCell{bg=gray!15} \cc{ws2$\blacktriangle$04} & \SetCell{bg=gray!15} vuln\_004 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/121.html}{121} & \SetCell{bg=gray!15} Stack-based Buffer Overflow \\
 &  &  & \cc{ws3$\blacktriangle$06} & vuln\_006 & \href{https://cwe.mitre.org/data/definitions/122.html}{122} & Heap-based Buffer Overflow \\
 &  &  & \SetCell{bg=gray!15} \cc{ws4$\blacktriangle$07} & \SetCell{bg=gray!15} vuln\_007 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/126.html}{126} & \SetCell{bg=gray!15} Buffer Over-read \\
 &  &  & \cc{ws5$\blacktriangle$08} & vuln\_008 & \href{https://cwe.mitre.org/data/definitions/129.html}{129} & Improper Validation of Array Index \\
 &  &  & \SetCell{bg=gray!15} \cc{ws7$\blacktriangle$13} & \SetCell{bg=gray!15} vuln\_013 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/120.html}{120} & \SetCell{bg=gray!15} Buffer Copy without Checking Size of Input ('Classic Buffer Overflow') \\
\cline{3-7}
 &  & xz & \cc{xz1$\square$01} & xz-001 & \href{https://cwe.mitre.org/data/definitions/416.html}{416} & Use After Free \\
\midrule
\SetCell[r=10]{m} \textbf{Java} & \SetCell[r=10]{} P1 & \SetCell[r=8]{} commons-compress & \SetCell[r=3]{bg=gray!15} \cc{cc1$\blacktriangle$03} & \SetCell[r=3]{bg=gray!15} vuln\_3 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/400.html}{400} & \SetCell{bg=gray!15} Uncontrolled Resource Consumption \\
 &  &  &  &  & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/770.html}{770} & \SetCell{bg=gray!15} Allocation of Resources Without Limits or Throttling \\
 &  &  &  &  & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/1333.html}{1333} & \SetCell{bg=gray!15} Inefficient Regular Expression Complexity \\
 &  &  & \SetCell[r=3]{} \cc{cc4$\blacktriangle$06} & \SetCell[r=3]{} vuln\_6 & \href{https://cwe.mitre.org/data/definitions/35.html}{35} & Path Traversal: '.../...//' \\
 &  &  &  &  & \href{https://cwe.mitre.org/data/definitions/22.html}{22} & Improper Limitation of a Pathname to a Restricted Directory ('Path Traversal') \\
 &  &  &  &  & \href{https://cwe.mitre.org/data/definitions/29.html}{29} & Path Traversal: '..filename' \\
 &  &  & \SetCell[r=2]{bg=gray!15} \cc{cc5$\blacktriangle$10} & \SetCell[r=2]{bg=gray!15} vuln\_10 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/77.html}{77} & \SetCell{bg=gray!15} Improper Neutralization of Special Elements used in a Command ('Command Injection') \\
 &  &  &  &  & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/28.html}{28} & \SetCell{bg=gray!15} Path Traversal: '..filedir' \\
\cline{3-7}
 &  & \SetCell[r=2]{} tika & \SetCell[r=2]{} \cc{tk6$\blacktriangle$10} & \SetCell[r=2]{} vuln\_10 & \href{https://cwe.mitre.org/data/definitions/834.html}{834} & Excessive Iteration \\
 &  &  &  &  & \href{https://cwe.mitre.org/data/definitions/407.html}{407} & Inefficient Algorithmic Complexity \\
\pagebreak
\cline{3-7}
\SetCell[r=35]{m} \textbf{Java} & \SetCell[r=33]{} P2 & \SetCell[r=6]{} commons-compress & \SetCell[r=3]{bg=gray!15} \cc{cc6$\blacktriangle$07} & \SetCell[r=3]{bg=gray!15} vuln\_7 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/35.html}{35} & \SetCell{bg=gray!15} Path Traversal: '.../...//' \\
 &  &  &  &  & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/22.html}{22} & \SetCell{bg=gray!15} Improper Limitation of a Pathname to a Restricted Directory ('Path Traversal') \\
 &  &  &  &  & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/29.html}{29} & \SetCell{bg=gray!15} Path Traversal: '..filename' \\
 &  &  & \SetCell[r=3]{} \cc{cc7$\blacktriangle$08} & \SetCell[r=3]{} vuln\_8 & \href{https://cwe.mitre.org/data/definitions/35.html}{35} & Path Traversal: '.../...//' \\
 &  &  &  &  & \href{https://cwe.mitre.org/data/definitions/22.html}{22} & Improper Limitation of a Pathname to a Restricted Directory ('Path Traversal') \\
 &  &  &  &  & \href{https://cwe.mitre.org/data/definitions/29.html}{29} & Path Traversal: '..filename' \\
\cline{3-7}
 &  & \SetCell[r=14]{} pdfbox & \SetCell[r=2]{bg=gray!15} \cc{pb1$\blacktriangle$02} & \SetCell[r=2]{bg=gray!15} vuln\_2 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/77.html}{77} & \SetCell{bg=gray!15} Improper Neutralization of Special Elements used in a Command ('Command Injection') \\
 &  &  &  &  & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/28.html}{28} & \SetCell{bg=gray!15} Path Traversal: '..filedir' \\
 &  &  & \SetCell[r=2]{} \cc{pb1$\square$00} & \SetCell[r=2]{} vuln\_0 & \href{https://cwe.mitre.org/data/definitions/611.html}{611} & Improper Restriction of XML External Entity Reference \\
 &  &  &  &  & \href{https://cwe.mitre.org/data/definitions/918.html}{918} & Server-Side Request Forgery (SSRF) \\
 &  &  & \SetCell[r=2]{bg=gray!15} \cc{pb1$\square$01} & \SetCell[r=2]{bg=gray!15} vuln\_1 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/611.html}{611} & \SetCell{bg=gray!15} Improper Restriction of XML External Entity Reference \\
 &  &  &  &  & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/918.html}{918} & \SetCell{bg=gray!15} Server-Side Request Forgery (SSRF) \\
 &  &  & \SetCell[r=2]{} \cc{pb1$\square$03} & \SetCell[r=2]{} vuln\_3 & \href{https://cwe.mitre.org/data/definitions/835.html}{835} & Loop with Unreachable Exit Condition ('Infinite Loop') \\
 &  &  &  &  & \href{https://cwe.mitre.org/data/definitions/834.html}{834} & Excessive Iteration \\
 &  &  & \SetCell[r=2]{bg=gray!15} \cc{pb1$\square$04} & \SetCell[r=2]{bg=gray!15} vuln\_4 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/835.html}{835} & \SetCell{bg=gray!15} Loop with Unreachable Exit Condition ('Infinite Loop') \\
 &  &  &  &  & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/834.html}{834} & \SetCell{bg=gray!15} Excessive Iteration \\
 &  &  & \cc{pb1$\square$05} & vuln\_5 & \href{https://cwe.mitre.org/data/definitions/789.html}{789} & Memory Allocation with Excessive Size Value \\
 &  &  & \SetCell{bg=gray!15} \cc{pb1$\square$06} & \SetCell{bg=gray!15} vuln\_6 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/789.html}{789} & \SetCell{bg=gray!15} Memory Allocation with Excessive Size Value \\
 &  &  & \cc{pb1$\square$07} & vuln\_7 & \href{https://cwe.mitre.org/data/definitions/834.html}{834} & Excessive Iteration \\
 &  &  & \SetCell{bg=gray!15} \cc{pb1$\square$08} & \SetCell{bg=gray!15} vuln\_8 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/834.html}{834} & \SetCell{bg=gray!15} Excessive Iteration \\
\cline{3-7}
 &  & \SetCell[r=13]{} poi & \cc{po1$\blacktriangle$05} & vuln\_5 & \href{https://cwe.mitre.org/data/definitions/918.html}{918} & Server-Side Request Forgery (SSRF) \\
 &  &  & \SetCell[r=2]{bg=gray!15} \cc{po1$\blacktriangle$06} & \SetCell[r=2]{bg=gray!15} vuln\_6 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/121.html}{121} & \SetCell{bg=gray!15} Stack-based Buffer Overflow \\
 &  &  &  &  & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/20.html}{20} & \SetCell{bg=gray!15} Improper Input Validation \\
 &  &  & \SetCell[r=2]{} \cc{po1$\square$00} & \SetCell[r=2]{} vuln\_0 & \href{https://cwe.mitre.org/data/definitions/834.html}{834} & Excessive Iteration \\
 &  &  &  &  & \href{https://cwe.mitre.org/data/definitions/20.html}{20} & Improper Input Validation \\
 &  &  & \SetCell[r=3]{bg=gray!15} \cc{po1$\square$01} & \SetCell[r=3]{bg=gray!15} vuln\_1 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/789.html}{789} & \SetCell{bg=gray!15} Memory Allocation with Excessive Size Value \\
 &  &  &  &  & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/770.html}{770} & \SetCell{bg=gray!15} Allocation of Resources Without Limits or Throttling \\
 &  &  &  &  & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/20.html}{20} & \SetCell{bg=gray!15} Improper Input Validation \\
 &  &  & \SetCell[r=2]{} \cc{po1$\square$02} & \SetCell[r=2]{} vuln\_2 & \href{https://cwe.mitre.org/data/definitions/35.html}{35} & Path Traversal: '.../...//' \\
 &  &  &  &  & \href{https://cwe.mitre.org/data/definitions/20.html}{20} & Improper Input Validation \\
 &  &  & \SetCell[r=2]{bg=gray!15} \cc{po1$\square$03} & \SetCell[r=2]{bg=gray!15} vuln\_3 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/695.html}{695} & \SetCell{bg=gray!15} Use of Low-Level Functionality \\
 &  &  &  &  & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/20.html}{20} & \SetCell{bg=gray!15} Improper Input Validation \\
 &  &  & \cc{po1$\square$04} & vuln\_4 & \href{https://cwe.mitre.org/data/definitions/382.html}{382} & J2EE Bad Practices: Use of System.exit() \\
\hline
 & \SetCell[r=2]{} P6 & \SetCell[r=2]{} logging-log4j2 & \SetCell[r=2]{bg=gray!15} \cc{lj1$\blacktriangle$00} & \SetCell[r=2]{bg=gray!15} vuln\_0 & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/917.html}{917} & \SetCell{bg=gray!15} Improper Neutralization of Special Elements used in an Expression Language Statement ('Expression Language Injection') \\
 &  &  &  &  & \SetCell{bg=gray!15} \href{https://cwe.mitre.org/data/definitions/20.html}{20} & \SetCell{bg=gray!15} Improper Input Validation \\
\bottomrule
\end{longtblr}
\twocolumn

==> tbl/vuln_sarif_details/sarif_broadcasts.tex <==
\begin{longtblr}[
  caption = {SARIF broadcast details. $\square$ indicates full-mode challenges, $\blacktriangle$ indicates delta-mode challenges.},
  label = {t:sarif-broadcast-details},
]{
  colspec = {l|llll},
  rows = {font=\footnotesize, abovesep=0pt, belowsep=-1pt},
  row{1} = {font=\bfseries\footnotesize, belowsep=1pt},
  rowhead = 1,
  colsep = 3pt,
}
\toprule\addlinespace[2pt]
Ph & Project & Lang & Label & Answer \\
\midrule
\SetCell[r=7]{} P2 & little-cms & C & \SetCell{bg=gray!15} \cc{cm1$\square$01} & \SetCell{bg=gray!15} CORRECT \\
\cline{2-5}
 & curl & C & \cc{cu3$\blacktriangle$$\ominus$} & INCORRECT \\
\cline{2-5}
 & libexif & C & \SetCell{bg=gray!15} \cc{ex2$\blacktriangle$$\ominus$} & \SetCell{bg=gray!15} INCORRECT \\
\cline{2-5}
 & freerdp & C & \cc{fp2$\blacktriangle$02} & CORRECT \\
\cline{2-5}
 & poi & Java & \SetCell{bg=gray!15} \cc{po1$\square$02} & \SetCell{bg=gray!15} CORRECT \\
\cline{2-5}
 & shadowsocks-libev & C & \cc{ss1$\square$00} & CORRECT \\
\cline{2-5}
 & systemd & C & \SetCell{bg=gray!15} \cc{sd1$\square$04} & \SetCell{bg=gray!15} CORRECT \\
\hline
\SetCell[r=1]{} P6 & logging-log4j2 & Java & \cc{lj1$\blacktriangle$00} & CORRECT \\
\hline
\SetCell[r=5]{} P7 & \SetCell[r=4]{} wireshark & \SetCell[r=4]{} C & \SetCell{bg=gray!15} \cc{ws1$\blacktriangle$03} & \SetCell{bg=gray!15} CORRECT \\
 &  &  & \cc{ws2$\blacktriangle$$\ominus$} & INCORRECT \\
 &  &  & \SetCell{bg=gray!15} \cc{ws3$\blacktriangle$$\ominus$} & \SetCell{bg=gray!15} INCORRECT \\
 &  &  & \cc{ws4$\blacktriangle$$\ominus$} & INCORRECT \\
\cline{2-5}
 & xz & C & \SetCell{bg=gray!15} \cc{xz1$\square$01} & \SetCell{bg=gray!15} CORRECT \\
\bottomrule
\end{longtblr}

==> tbl/vuln_sarif_details/zerodays.tex <==
\begin{longtblr}[
  caption = {0-day vulnerabilities discovered during the competition. $\square$ indicates full-mode challenges, $\blacktriangle$ indicates delta-mode challenges.},
  label = {t:zeroday-details},
]{
  colspec = {c|l|llX[l]},
  rows = {font=\scriptsize, abovesep=0pt, belowsep=-1pt},
  row{1} = {font=\bfseries\scriptsize, belowsep=1pt},
  rowhead = 1,
  colsep = 3pt,
}
\toprule\addlinespace[2pt]
Lang & Ph & Project & ID & Description \\
\midrule
\SetCell[r=10]{m} \textbf{C} & \SetCell[r=9]{} P2 & little-cms & \SetCell{bg=gray!15} \cc{cm1$\square$a} & \SetCell{bg=gray!15} UBSan: Signed integer overflow \\
\cline{3-5}
 &  & \SetCell[r=3]{} curl & \cc{cu5$\blacktriangle$a} & ASan: Heap buffer overflow \\
 &  &  & \SetCell{bg=gray!15} \cc{cu5$\blacktriangle$b} & \SetCell{bg=gray!15} ASan: Abort signal \\
 &  &  & \cc{cu5$\blacktriangle$c} & ASan: Segmentation fault \\
\cline{3-5}
 &  & mongoose & \SetCell{bg=gray!15} \cc{mg1$\square$a} & \SetCell{bg=gray!15} ASan: Memory leak \\
\cline{3-5}
 &  & \SetCell[r=3]{} shadowsocks-libev & \cc{ss1$\square$a} & UBSan: Signed integer overflow \\
 &  &  & \SetCell{bg=gray!15} \cc{ss1$\square$b} & \SetCell{bg=gray!15} UBSan: Signed integer overflow \\
 &  &  & \cc{ss1$\square$c} & UBSan: Signed integer overflow \\
\cline{3-5}
 &  & systemd & \SetCell{bg=gray!15} \cc{sd1$\square$a} & \SetCell{bg=gray!15} ASan: Abort signal \\
\hline
 & \SetCell[r=1]{} P3 & wireshark & \cc{ws1$\square$a} & ASan: Stack buffer overflow \\
\midrule
\SetCell[r=15]{m} \textbf{Java} & \SetCell[r=15]{} P2 & {healthcare-data-\\harmonization} & \SetCell{bg=gray!15} \cc{hc1$\square$a} & \SetCell{bg=gray!15} Stack overflow \\
\cline{3-5}
 &  & hertzbeat & \cc{hb1$\square$a} & Out of memory \\
\cline{3-5}
 &  & \SetCell[r=9]{} pdfbox & \SetCell{bg=gray!15} \cc{pb1$\blacktriangle$a} & \SetCell{bg=gray!15} Stack overflow \\
 &  &  & \cc{pb1$\blacktriangle$b} & Out of memory \\
 &  &  & \SetCell{bg=gray!15} \cc{pb1$\blacktriangle$c} & \SetCell{bg=gray!15} Stack overflow \\
 &  &  & \cc{pb1$\square$d} & Out of memory \\
 &  &  & \SetCell{bg=gray!15} \cc{pb1$\square$e} & \SetCell{bg=gray!15} Stack overflow \\
 &  &  & \cc{pb1$\square$f} & Stack overflow \\
 &  &  & \SetCell{bg=gray!15} \cc{pb1$\square$g} & \SetCell{bg=gray!15} Class not found \\
 &  &  & \cc{pb1$\square$h} & Stack overflow \\
 &  &  & \SetCell{bg=gray!15} \cc{pb1$\square$i} & \SetCell{bg=gray!15} Stack overflow \\
\cline{3-5}
 &  & \SetCell[r=4]{} poi & \cc{po1$\square$a} & Out of memory \\
 &  &  & \SetCell{bg=gray!15} \cc{po1$\square$b} & \SetCell{bg=gray!15} Out of memory \\
 &  &  & \cc{po1$\square$c} & Stack overflow \\
 &  &  & \SetCell{bg=gray!15} \cc{po1$\square$d} & \SetCell{bg=gray!15} Out of memory \\
\bottomrule
\end{longtblr}
